A Unified Framework of Light Spanners II: Fine-Grained Optimality

Seminal works on light spanners over the years provide spanners with optimal lightness in various graph classes, such as in general graphs, Euclidean spanners, and minor-free graphs. Three shortcomings of previous works on light spanners are: (1) The techniques are ad hoc per graph class, and thus can't be applied broadly. (2) The runtimes of these constructions are almost always sub-optimal, and usually far from optimal. (3) These constructions are optimal in the standard and crude sense, but not in a refined sense that takes into account a wider range of involved parameters. This work aims at addressing these shortcomings by presenting a unified framework of light spanners in a variety of graph classes. Informally, the framework boils down to a transformation from sparse spanners to light spanners; since the state-of-the-art for sparse spanners is much more advanced than that for light spanners, such a transformation is powerful. Our framework is developed in two papers. The current paper is the second of the two -- it builds on the basis of the unified framework laid in the first paper, and then strengthens it to achieve more refined optimality bounds for several graph classes. Among various applications and implications of our framework, we highlight here the following: For $K_r$-minor-free graphs, we provide a $(1+\epsilon)$-spanner with lightness $\tilde{O}_{r,\epsilon}( \frac{r}{\epsilon} + \frac{1}{\epsilon^2})$, improving the lightness bound $\tilde{O}_{r,\epsilon}( \frac{r}{\epsilon^3})$ of Borradaile, Le and Wulff-Nilsen. We complement our upper bound with a lower bound construction, for which any $(1+\epsilon)$-spanner must have lightness $\Omega(\frac{r}{\epsilon} + \frac{1}{\epsilon^2})$. We note that the quadratic dependency on $1/\epsilon$ we proved here is surprising, as the prior work suggested that the dependency on $\epsilon$ should be $1/\epsilon$.

==> Opt-Stretch-t.tex <==

\section{Optimal Light Spanners for Stretch $t\geq 2$}\label{sec:unified}



In this section, we present a construction of light spanners from sparse spanner oracles with stretch $t \geq 2$. Here we focus more on achieving on optimizing for the dependency on $\epsilon$. 

\begin{theorem}\label{thm:cluster-opt-t2}
	Let $\psi = 1$ and $\zeta = 1/250$. There is an algorithm that can find a subgraph $\mathcal{H}_i\subseteq \tilde{G}$ and construct clusters in $\mathcal{C}_{i+1}$  such that:
	\begin{equation*}
	w(H_i) = O( \frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon}) \Delta^i_{L} +  O(L_i)
	\end{equation*}
and that $d_{H_{\leq i}}(u,v) \leq t(1+\epsilon)d_G(u,v)$ for every edge $(u,v)\in E_i$. 
\end{theorem}

The value of $\zeta $ in Theorem~\ref{thm:cluster-opt-t2} is somewhat arbitrary; any value sufficiently smaller than $1$ works. We first show that Theorem~\ref{thm:cluster-opt-t2} implies Theorem~\ref{thm:general-stretch-2}. 

\begin{proof}[Proof of Theorem~\ref{thm:general-stretch-2}] Observe that Theorem~\ref{thm:cluster-opt-t2} implies Lemma~\ref{lm:potential-reduction} with $\lambda = O(\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon})$ and $a_i = O(L_i)$.  We observe that: 
	\begin{equation}\label{eq:A-bound-stretch-2}
	\begin{split}
	A &= \sum_{i=1}^{I}a_i =\sum_{i=1}^{I}O(L_i)=  O(1) \sum_{i=1}^{I} \frac{L_I}{\epsilon^{I-i}} = O(\frac{L_I}{1-\epsilon}) = O(1) w(\mst) 
	\end{split}
	\end{equation}
	since $L_i\leq w(\mst)$ and $\epsilon\leq \frac{1}{2}$. Thus, we can construct a $t(1+\epsilon)$-spanner with lightness:
	\begin{equation}
	O(\frac{1}{\psi}(\frac{ \wsp_{\mathcal{O}_{G,t}}}{\epsilon} +  1)\log\frac{1}{\epsilon}) = \tilde{O}_{\epsilon}(\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon})
	\end{equation}
	since $\psi = 1$; this completes Theorem~\ref{thm:general-stretch-2}.\qed
\end{proof}

\subsection{High Level Ideas}\label{subsec:highLevel-t2}

In this section, we describe high-level ideas of the construction in Theorem~\ref{thm:cluster-opt-t2}. While it is not required to read the cluster construction in Section~\ref{sec:fast-general} to understand the construction in this section, we recommend the readers to do so for two reasons. First, it is much simpler. (However, the dependency on $\epsilon$ is $\frac{1}{\epsilon^4}$.) Second, it is a starting point for us to reduce the dependency on $\epsilon$, from $\frac{1}{\epsilon^4}$ all the way down to $\frac{1}{\epsilon}$. We observe that one $\frac{1}{\epsilon}$ factor is due to $\psi = \epsilon$.  Thus, by chosing $\psi = 1$ in Theorem~\ref{thm:cluster-opt-t2}, we already reduce the dependency on $\epsilon$ from $\frac{1}{\epsilon^4}$ to $\frac{1}{\epsilon^3}$.

The construction has five steps (instead of four steps as in Section~\ref{sec:fast-general}). The intuition for each step remains the same: superclusters are constructed in a way that the local potential reduction is as large as possible. We again distinguish between \emph{heavy clusters} and \emph{light clusters}: heavy clusters are incident to at least $\frac{2g}{\epsilon}$ edges in $\me_i$ while light clusters are incident to less than $\frac{2g}{\epsilon}$ edges.  

In Step 1, we group all heavy clusters into superclusters. It can be shown that (see Lemma~\ref{lm:Step1Weight}) each Step-1 supercluster $\mx$ has local potential reduction $\Delta^i_{L}(\mx) = \Omega(|\mv(\mx)|\epsilon L_i)$. If one calls the sparse spanner oracles  on \emph{heavy} nodes and  take all edges incident to light nodes clustered in Step 1 to $H_i$, the total weight will be $O(\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon} + \frac{1}{\eps^2})$  times the total potential reduction. This means that the final lightness must depend at least quadratically on $\frac{1}{\epsilon}$ while we want a linear dependency on $\frac{1}{\epsilon}$. 

Observe that the additive $+\frac{1}{\epsilon^2}$ is due to the fact that each light node is incident up to $\Omega(\frac{1}{\epsilon})$ level-$i$ edges of weight  $\Theta(L_i)$ each, while it only has $O(\epsilon L_i)$ unit of  potential reduction (if we evenly distribute the potential reduction of $\mx$ to every node in $\mx$). Thus, we need to somehow reduce the number of incident edges of lightness to $O(1)$. 

Our key idea is to not restrict the construction of sparse spanner oracles to only heavy nodes. Instead,  we will select a \emph{subset of light nodes} and construct the oracle on both heavy nodes and the selected subset of light nodes. We then can show that for remaining light nodes, while the worst-case bound on the number of incident edges remains $\Theta(\frac{1}{\epsilon})$, the average number of incident edges is just $O(1)$. To identify the subset of light nodes in Step 5, we rely on the structures of superclusters  in previous steps. As a result, the construction of sparse spanner oracles will be delayed until Step 5. 

In Step 2, we group (a subset of) \emph{branching} nodes, whose degree in the spanning tree $\widetilde{\mst}_i$ is at least $3$, into superclusters (which are subtrees of $\widetilde{\mst}_i$).  The main observation is that any supercluster that is a subtree of $\widetilde{\mst}_i$ with at least \emph{one} branching node will have positive potential reduction --  this is because at least one neighbor of a branching node will not belong to the diameter path. More precisely, if $\mx$ is such a cluster, then $\Delta^i_{L}(\mx) \geq \Omega(|\mv(\mx)|\epsilon^2 L_i )$, as shown in Lemma~\ref{lm:Step2Cluster}. However, this would incur lightness $O(\frac{1}{\epsilon^2})$, assuming that light nodes incident to $O(1)$ edges by applying ideas sketched in the previous paragraph. 

Our idea is to boost the potential reduction to $\Omega(|\mv(\mx)|\epsilon L_i )$ by clustering branching nodes into small superclusters, those of augmented diameter at most $2\zeta L_i$ in such a way that small clusters with an augmented diameter at least $\zeta L_i$ will have $\Omega(\frac{1}{\epsilon})$ nodes that do not belong to the diameter path. We use the tree clustering procedure given in our prior work~\cite{LS19} in the analysis of the greedy algorithm for \emph{geometric spanners} to accomplish this.

In Step 3, we cluster edges in $\me_i$ whose endpoints are far from each other. The construction is similar to Step 3 in Section~\ref{sec:fast-general}; each supercluster $\mx$ has $\Omega(|\mv(\mx)|\epsilon L_i)$  amount  potential reduction.   In Step 4, we break long paths into smaller subpaths and form superclusters from these subpaths. Superclusters in Step 4 may have zero potential reduction, and the key idea is to show that potential reduction of superclusters in previous steps can bound the total weight of edges incident to Step-4 superclusters. 

In Step 5, we re-group superclusters formed in previous steps into bigger superclusters. The idea, as discussed in Step 1, is to identify a subset of light nodes on which, together with heavy nodes, we construct a sparse spanner oracle. For remaining light nodes, we are able to show that, on average, they are incident to only $O(1)$ edges. Thus, the total weight of them is at most $O(\frac{1}{\epsilon})$ time the total potential reduction, which incurs lightness $O(\frac{1}{\epsilon})$. We are now ready to give the full details of the construction.


\subsection{Proof of Theorem~\ref{thm:cluster-opt-t2}}




Recall that $\mg_i(\mv_i, \me_i \cup \widetilde{\mst}_i,\omega)$ is a cluster graph with edges in $\widetilde{\mst}_i$ is a spanning tree of $\mg$ (see Lemma~\ref{lm:spanning-Gi}). We will construct a set of superclusters $\mx$, which are subgraphs of $\mg_i$; $\varphi(\mx)$ will then be a level-$(i+1)$ clusters. 


  Let $\mathcal{K}_i (\mathcal{V}_i, \mathcal{E}_i)$ be the spanning subgraph of $\mg_i$ induced by $\me_i$.    For each node $\nu$, we denote by $\mathcal{E}_i(\nu)$ the set of edges incident to $\nu$ in $\mathcal{K}_i$. We call a node $\nu$ of $\mathcal{K}_i$ \emph{heavy} if $|\mathcal{E}_i(\nu)| \geq \frac{2g}{\zeta\epsilon}$ and \emph{light} otherwise\footnote{We have an additional $\zeta$ factor in the definition of heavy nodes compared to the definition in Subsection~\ref{subsec:fast-clustering}.}. Let $\mathcal{V}_{hv}$ ($\mathcal{V}_{li}$)  be the set of heavy (light) nodes. Let $\mathcal{V}^+_{hv} = \mathcal{V}_{hv} \cup N_{\mathcal{K}_i}[\mathcal{V}_{hv}]$ and $\mathcal{V}^-_{li} = \mathcal{V}_i \setminus \mathcal{V}^+_{hv}$.


\paragraph{Step 1.~} In the first step, we group all nodes in $\mathcal{V}^+_{hv}$ into  superclusters. We use the same construction in Steps 1A and 1B in  Section~\ref{subsec:fast-clustering}, that we reproduce here for completeness.



\begin{itemize}
	\item \textbf{Step 1A.~} This step has two mini-steps. (See Figure~\ref{fig:K-graph}.)
	
	\begin{itemize}
		\item (Step 1A(i).~)  Let $\mathcal{I}\subseteq \mathcal{V}_{hv}$ be a maximal 2-hop independent set over the nodes of $\mathcal{V}_{hv}$, which in particular guarantees that $\nu,\mu \in \mathcal{I}$, $N_{\mathcal{K}_i}[\nu] \cap N_{\mathcal{K}_i}[\mu] = \emptyset$.  For each node $\nu \in \mathcal{I}$, form a supercluster $\mx$ from $\nu$, $\nu$'s neighbors and incident edges, and add to $H_i$ the edge set $\mathcal{E}_i(v)$\footnote{To be precise, we add to $H_i$ the sources of edges in $\mathcal{E}_i(v)$.}. We then designate any node in $\mx$ as its representative.
		\item (Step 1A(ii).~) We iterate over the nodes of $\mathcal{V}_{hv}\setminus \mathcal{I}$ that are not grouped yet to any supercluster. For each such node  $\mu \in \mathcal{V}_{hv}\setminus \mathcal{I}$, there must be a neighbor $\mu'$ that is already grouped to a supercluster, say $\mx$; if there are multiple such vertices, we pick one of them arbitrarily. We add $\mu$ and edge $(\mu,\mu')$ to $\mathcal{X}$, and add $(\mu,\mu')$ to $H_i$. Observe that every heavy node is grouped at the end of this step.
	\end{itemize}
	
	\item  \textbf{Step 1B.~} For each node $\nu$ in $\mathcal{V}^+_{hv}$ that is not grouped in Step 1, there must be at least one neighbor, say $\mu$, of $\nu$ grouped in Step 1; if there are multiple such nodes, we pick one of them arbitrarily. We add $\mu$ and the edge $(\nu,\mu)$ to the supercluster containing $\nu$. We then add edge $(\nu,\mu)$ to $H_i$.
\end{itemize}


\noindent Superclusters in Step 1 have the following property; the proof is the same as the proof of Lemma~\ref{lm:3-steps}.


\begin{lemma}\label{lm:Step1-Diam-Oracle} Every supercluster  $\mx$ formed  in Step 1   has: (a) $\varphi(\mx)\subseteq H_{\leq i}$, (b) $L_{i}\leq \adm(\mx)\leq 13L_{i}$  and (c) at least $\frac{2g}{\epsilon} $ nodes.
\end{lemma}
\begin{proof}[Sketch] Property (a) follows from induction and the fact that  every level-$i$ edge in $\mx$ is added to $H_i$. Property (c) follows from that every Step 1 supercluster contains a heavy node and \emph{all of its neighbors} by the construction in Step 1A. Property (b) follows from two facts: (i) every node has weight at most $g\epsilon L_i$  and (ii) $\mx$ has hop diameter at most $6$ (see Figure~\ref{fig:K-graph}).  In bounding $\adm(\mx)$, we assume that $\epsilon \ll \frac{1}{g}$. \qed
\end{proof}

	\begin{wrapfigure}{r}{0.4\textwidth}
	\vspace{-25pt}
	\begin{center}
		\includegraphics[width=0.35\textwidth]{K-graph}
	\end{center}
	\caption{\footnotesize{Superclusters formed in Step 1. Yellow nodes are heavy nodes. The green-shaded superclusters are formed in Step 1A(i); superclusters enclosed by purple dashed curves are formed in Step 1A(ii); superclusters enclosed by blue dashed curves, which become level-$1$ superclusters, are formed in Step 1B. }}
	\vspace{-20pt}
	\label{fig:K-graph}
\end{wrapfigure}

\paragraph{Required definitions/preparations for Step 2.~} Recall by Lemma~\ref{lm:spanning-Gi} that $\widetilde{\mst}_i$ induces a spanning tree of $\mathcal{G}_i$. Let $\mathcal{F}_1$ be the forest of level-$i$ clusters after Step 1 -- nodes of $\mathcal{F}_1$ are unclustered light nodes of $\mathcal{K}_i$, and edges of $\mathcal{F}_1$ are edges in $\widetilde{\mst}_i$. We call a node  \emph{$\mt$-branching} if it has at least degree 3 in  a tree $\mt$. We will simply say a node \emph{branching} when the tree is clear from the context. 


Our goal in this step is to cluster nodes in such a way that each supercluster has a large potential reduction. To this end, we make use of the following construction (Lemma~\ref{lm:tree-clustering} below) in~\cite{LS19} as a preprocessing. 

For each node $\alpha\in \mf_1$, let $B_{\mf_1}(\alpha, r)$ be the subtree of $\mf_1$ induced by \emph{all nodes} of augmented distance at most $r$ from $\alpha$. 


\begin{lemma}[Section 6.3.2 in~\cite{LS19}]\label{lm:tree-clustering} Let $\mt$ be a tree with vertex weight and edge weight. Let $L, \eta, \gamma$ be three parameters where $\eta \ll \gamma \ll 1$. Suppose that for any vertex $v\in \mt$ and any edge $e\in \mt$, $w(e) \leq w(v) \leq \eta L$. There is a polynomial-time algorithm that finds a collection of vertex-disjoint subtrees $\mathbb{U} = \{\mt_1,\ldots, \mt_k\}$ of $\mt$ such that:
	\begin{enumerate}
		\item[(1)] $\adm(\mt_i) \leq 2\gamma L$ for any $1\leq i \leq k$.
		\item[(2)] Every branching node is contained in some tree in $\mathbb{U}$. 
		\item[(3)] Each tree $\mt_i$ contains a $\mt_i$-branching node $\beta_i$ and three node-disjoint paths $\mp_1,\mp_2, \mp_3$ that have $\beta_i$ as the same endpoint, such that $\adm(\mp_1\cup \mp_2) = \adm(\mt_i)$ and $\adm(\mp_3 \setminus \{\beta_i\})= \Omega(\adm(\mt_i))$. We call $\beta_i$ the \emph{center} of $\mt_i$.
		\item[(4)] Let $\overline{\mt}$ be obtained by contracting each subtree of $\mathbb{U}$ into a single node. Then each $\overline{\mt}$-branching node corresponds to a sub-tree  of augmented diameter at least $\gamma L$.
	\end{enumerate}
\end{lemma}

	\begin{wrapfigure}{r}{0.4\textwidth}
	\vspace{-20pt}
	\begin{center}
		\includegraphics[width=0.4\textwidth]{T-clustering}
	\end{center}
	\caption{\footnotesize{(a) A collection $\mathbb{U} = \{\mt_1,\mt_2,\mt_3\}$ of a tree $\mt$ as in Lemma~\ref{lm:tree-clustering}. Yellow nodes are $\mt$-branching nodes. Big yellow nodes are the centers of their corresponding subtrees in $\mathbb{U}$. (b)  The shaded node in $\overline{\mt}$ is a $\overline{\mt}$-branching node and has an augmented diameter of at least $\gamma L$.}}
	\vspace{-40pt}
	\label{fig:T-clustering}
\end{wrapfigure}


\noindent See an illustration of Lemma~\ref{lm:tree-clustering}  in Figure~\ref{fig:T-clustering}. We are now ready to describe Step 2.


\begin{itemize}
	\item \textbf{Step 2} For every tree $\mathcal{T}\in \mathcal{F}_1$ of augmented diameter at least $\zeta L_i$,   we construct a collection of subtree $\mathbb{U}_\mathcal{T} = \{\mathcal{T}_1, \ldots, \mathcal{T}_k\}$ of $\mathcal{T}$ using Lemma~\ref{lm:tree-clustering} with $\eta = g\epsilon$ and $\gamma = \zeta$. For each subtree $\mathcal{T}_j \in \mathbb{U}_{\mathcal{T}}$ where $j\in [1,k]$, if $\adm(\mathcal{T}_j)\geq \zeta L_i$, we make $\mathcal{T}_j$ a supercluster. (See Figure~\ref{fig:Step2-opt}(a).) 
\end{itemize}


The key property of superclusters in Step 2 is that each supercluster $\mx$ has a local pontential reduction $\Delta_{L}^i(\mx) = \Omega(|\mv(\mx)|\epsilon L_i)$ (see Lemma~\ref{lm:Step2ClusterOracle}).

\begin{lemma}\label{lm:Step2-Oracle-Diameter} 
	Every supercluster $\mx$ formed in Step 2 has: (a) $\varphi(\mx)\subseteq H_{\leq i}$, (b) $\zeta L_i \leq \adm(\mx)\leq 2\zeta L_i$  and (c) $|\mv(\mx)| = \Omega(\frac{1}{\epsilon})$ when $\epsilon \ll \frac{1}{g}$.
\end{lemma}
\begin{proof}
	 Observe that $\mx$ is a subtree of $\widetilde{\mst}_i$ and by induction, every node $\nu \in \mx$ has $\varphi(\nu) \subseteq H_{\leq i-1}$. Thus, $\varphi(\mx)\subseteq H_{\leq i-1}\subseteq H_{\leq i}$. The lower bound on the augmented diameter follows directly from the construction  and the upper bound follows from  Item (1) of Lemma~\ref{lm:tree-clustering}. 
	
		Let $\md$ be the diameter path of $\mx$; $\adm(\md)\geq \zeta L_i$ by construction. Since every edge has a weight at most $\bar{w} \leq L_{i-1}$ and each node has a weight in $[L_{i-1},g\epsilon L_{i-1}]$, $\md$ has at least $\frac{\adm(\md)}{2g\epsilon L_{i-1}} = \Omega(\frac{1}{\epsilon})$ nodes. This implies $|\mv(\mx)| = \Omega(\frac{1}{\epsilon})$. \qed
\end{proof}




\begin{figure}[hbt]
	\centering
	%\vspace{-20pt}
	\includegraphics[scale = 0.9]{Step2-opt}
	\caption{ \footnotesize{(a) Forest $\mf_1$. Yellow nodes are branching nodes. Nodes enclosed in dashed red curves are subtrees obtained by applying Lemma~\ref{lm:tree-clustering} to $\mf_1$. Shaded subtrees have augmented diameter at least $\zeta L_i$. (b) Forest $\overline{\mf}_2$. Big nodes are non-trivial supernodes. }}
	\label{fig:Step2-opt}
\end{figure}

\paragraph{Required definitions/preparations for Step 3.~} Let $\overline{\mathcal{F}_2}$ be the forest obtained from $\mathcal{F}_1$ as follows. For each tree $\mathcal{T} \in \mathcal{F}_1$, let $\bar{\mathbb{U}}_{\mathcal{T}}\subseteq \mathbb{U}_{\mathcal{T}}$ be the set of subtrees that are unclustered in Step 2. Let $\bar{\mathbb{U}}_{\mathcal{F}_1} = \cup_{\mathcal{T} \in \mathcal{F}_1}\bar{\mathbb{U}}_{\mathcal{T}}$. $\overline{\mathcal{F}_2}$ is obtained from $\mathcal{F}_1$ by (1) removing every clustered node in Step 2 from $\mathcal{F}_1$ and (2) contracting each subtree $\mathcal{T}' \in \bar{\mathbb{U}}_{\mathcal{F}_1}$ into a single node, called \emph{non-trivial supernode}.  We refer to the remaining nodes in $\overline{\mathcal{F}_2}$, which are nodes in $\mf_1$, as \emph{trivial supernodes}.  (See Figure~\ref{fig:Step2-opt}(b).)

For each supernode $\bar{\nu}\in \overline{\mf_2}$, we denote the subtree of $\mf_1$ corresponding to $\bar{\nu}$ by $\mt_{\bar{\nu}}$; if $\bar{\nu}$ is trivial, then $\mt_{\bar{\nu}}$ contains a single node $\nu$. We assign weight to each supernode as follows:
\begin{quote}
	\textbf{Supernode weight:} each supernode $\bar{\nu}$ is assigned a weight $\omega(\bar{\nu}) = \adm(\mt_{\bar{\nu}})$.
\end{quote}

The augmented diameter of each tree in $\overline{\mathcal{F}_2}$ is measured w.r.t edge and supernode weights.  

\begin{claim}\label{clm:BarF2-structure} Every tree in $\overline{\mathcal{F}_2}$ of augmented diameter at least $\zeta L_i$ is a path.
\end{claim}
\begin{proof}
	Let $\overline{\mathcal{T}}$ be a tree of $\overline{\mathcal{F}_2}$ of augmented diameter at least $\zeta L_i$. Suppose that $\overline{\mathcal{T}}$ has a branching node, say $\bar{\nu}$. By Item (2) in Lemma~\ref{lm:tree-clustering}, $\bar{\nu}$ must be node contracted from some tree in $\bar{\mathbb{U}}_{\mf_1}$. By Item (4) in Lemma~\ref{lm:tree-clustering}, the augmented diameter of  $\mathcal{T}_{\bar{\nu}}$ must be at least $\zeta L_i$. However, by the construction of Step 2, $\mathcal{T}_{\bar{\nu}}$ will be clustered and hence removed in the construction of $\overline{\mathcal{F}_2}$; this contradicts that $\bar{\nu}$ is in $\overline{\mathcal{F}_2}$.\qed
\end{proof}


Step 3 is applied to $\overline{\mathcal{F}_2}$.  We call  paths in $\overline{\mathcal{F}_2}$ of augmented diameter  at least $\zeta L_i$ \emph{long paths}.  For each long path $\overline{\mathcal{P}} \in \mathcal{F}_2$, we color their supernodes red or blue:  a supernode has an augmented distance at most $L_i$ from at least one of the endpoints of $\overline{\mathcal{P}}$ has a blue color and otherwise, it has  a red color. It could be that every node in $\overline{\mathcal{P}}$ is colored red.

For each blue supernode $\bar{\nu}$ of $\overline{\mathcal{P}}$, we assign a subpath $\overline{\mathcal{I}}(\bar{\nu})$ of $\overline{\mathcal{P}}$,
called the \emph{interval of $\bar{\nu}$}, which contains \emph{all supernodes} within augmented distance (in $\overline{\mathcal{P}}$) at most $L_i$ from $\bar\nu$. 
\begin{claim}\label{clm:Interval-node-unified}
	For any blue supernode $\bar\nu$, $ (2 - (3\zeta+2\epsilon))L_i  \leq  \adm(\overline{\mathcal{I}}(\bar\nu))\leq 2L_i $.
\end{claim}
\begin{proof} The proof is similar to that of Claim~\ref{clm:Interval-node}; we sketch the argument here. The upper bound on the augmented diameter of $\bar{\mi}(\bar{\nu})$ follows directly from the construction. For the lower bound, observe that supernodes  adjacent to the endpoints of $\bar{\mi}(\bar{\nu})$  are in augmented distance at least $L_i$ from $\bar{\nu}$. Excluding the weight of these supernodes (each of weight at most $\zeta L_i$) and the weight of two $\widetilde{\mst}_i$ edges (each of weight at most $\epsilon L_i$)  connecting them to the endpoints of $\bar{\nu}$, we have: 
\begin{equation*}
\adm(\bar{\mi}(\bar{\nu})) \geq 2(1- (\zeta + \epsilon) L_i)  - \omega(\bar\nu) \geq 2-(3\zeta+2\epsilon)L_i,
\end{equation*}
as desired.\qed 	
\end{proof}

We define the following two sets of edges with both blue endpoints (see Figure~\ref{fig:Step3-opt}):
\begin{equation}\label{eq:Bfar-Bclose}
\begin{split}
\mathcal{B}_{far} &= \{(\bnu,\bmu) \in \mathcal{E}_i \setminus H_i~|~ color(\bnu) = color({\bmu}) = blue  \mbox{ and } \overline{\mathcal{I}}(\bnu)\cap \mathcal{I}(\bmu) = \emptyset\}\\
\mathcal{B}_{close} &= \{(\bnu,\bmu) \in \mathcal{E}_i \setminus H_i~|~ color(\bnu) = color({\bmu}) = blue  \mbox{ and }\overline{\mathcal{I}}(\bnu)\cap \overline{\mathcal{I}}(\bmu) \not= \emptyset\}\\
\end{split}
\end{equation}

	\begin{wrapfigure}{r}{0.4\textwidth}
	\vspace{-25pt}
	\begin{center}
		\includegraphics[width=0.4\textwidth]{Step3-opt}
	\end{center}
	\caption{\footnotesize{Triangular nodes are non-trivial supernodes. The dashed red edge is in $\mb_{close}$ and the solid red edge is in $\mb_{far}$. $\overline{\mx}$ is the green-shaded region.}}
	\vspace{-25pt}
	\label{fig:Step3-opt}
\end{wrapfigure}

\begin{itemize}
	\item \textbf{Step 3.~}Pick an edge $ (\bar\nu,\bar\mu) \in \mathcal{B}_{far}$
	and form a supercluster $\bar{\mx} = \{(\bnu,\bmu)\cup \overline{\mathcal{I}}(\bnu) \cup \overline{\mathcal{I}}(\bmu)\}$.  We then add  $(\bar\nu,\bar\mu)$ to $H_i$. Let $\mx$ be obtained from $\bar{\mx}$ by uncontracting supernodes; we then regard $\mx$ as a Step-3 supercluster. Finally, we remove  all supernodes in  $\overline{\mathcal{I}}(\bnu) \cup \overline{\mathcal{I}}(\bmu)$ from the path or two paths containing $\bar\nu$ and $\bmu$; update the color of  supernodes in the new paths,  the edge sets $\mathcal{B}_{far}$ and  $\mathcal{B}_{close}$; and repeat this step until it no longer applies. (See Figure~\ref{fig:Step3-opt}.)
\end{itemize}


\begin{lemma}\label{lm:Step3-Diam-Oracle}
	Every supercluster $\mx$ formed in Step 3 has: (a) $\varphi(\mx)\subseteq H_{\leq i}$, (b) $L_i/2 \leq \adm(\mx)\leq 5L_i$  and (c) $|\mv(\mx)| = \Omega(\frac{1}{\epsilon})$ when $\epsilon \ll \frac{1}{g}$.
\end{lemma}
\begin{proof}
	Let $\bar{\mx}$ be the supercluster of supernodes corresponding to $\mx$.  By induction, each supernode $\bar{\nu}$ of $\bar{\mx}$ has $\varphi(\bar{\nu}) \subseteq H_{\leq i-1}$. Since we add edge $(\bar{\nu},\bar{\mu})$ to $H_i$ by construction, we have $\varphi(\mx)\subseteq H_{\leq i}$. 
	
	Observe by Claim~\ref{clm:Interval-node}  that $\bar{\mi}(\bar{\nu})$ has augmented diameter at most $2L_i$ and hence the uncontracted counterpart $\mi(\nu)$ obtained from $\bar{\mi}(\bar{\nu})$ by uncontracting nontrivial supernode has $\adm(\mi(\nu)) \leq \adm(\bar{\mi}(\bar{\nu}))\leq 2L_i$. Thus, $\adm(\mx) \leq \omega(\bnu,\bmu) + 2\cdot 2L_i \leq 5L_i$.	For the lower bound, we observe that $\adm(\mx)\geq \omega(\bnu,\bmu) \geq L_i/2$. 
	
By the same argument in the proof of Lemma~\ref{lm:Step2-Oracle-Diameter}, $|\mv(\mi(\nu))|  = \Omega(\frac{1}{\epsilon})$. Thus, $|\mv(\mx)| = \Omega(\frac{1}{\epsilon})$.	\qed
\end{proof}


\paragraph{Required definitions/preparations for Step 4.~}   Let $\overline{\mathcal{F}_3}$ be $\overline{\mathcal{F}_2}$ after Step 3; this step is similar to the construction of Step 4 in Subsection~\ref{subsec:fast-clustering}. There are two mini-steps: in Step 4A, we augment trees of low augmented diameter to existing superclusters, while in Step 4B, we break long paths into short subpaths, each of which becomes a supercluster.


\begin{itemize}
	\item \textbf{Step 4.~}  First, we discard all edges in $\mb_{close}$ and never consider them again in the following construction. 	Let $\overline{\mathcal{T}}$ be a tree of $\overline{\mathcal{F}_3}$; observe that there must be an $\widetilde{\mst}_i$ edge connecting $\overline{\mathcal{T}}$ to a supernode clustered in previous steps since $\widetilde{\mst}_i$ is a spanning tree. Let $\mt$ be the tree obtained from $\overline{\mathcal{T}}$  by uncontracting non-trivial supernodes; we call $\mt$ the \emph{uncontracted counterpart} of $\overline{\mt}$.
\begin{itemize}
	\item (Step 4A)  If $\adm(\mt)\leq \zeta L_i$, let $e$ be an $\widetilde{\mst}_i$ edge connecting $\mt$  and a node in a supercluster $\mx$. We add both $e$ and $\mt$ to $\mx$. 
	\item (Step 4B) 	Otherwise,  the augmented diameter of $\overline{\mathcal{T}}$ is at least $\zeta L_i$ and hence, it must be a path by Claim~\ref{clm:BarF2-structure}. In this case, we greedily break $\overline{\mathcal{T}}$ into a collection of subpaths, say $\overline{\mathbb{P}} = \{\overline{\mp}_1, \ldots, \overline{\mp}_t\}$ of augmented diameter at least $5\zeta L_i$ and at most $12\zeta L_i$ as follows. 
	\begin{itemize}
		\item[] 	Initially $\overline{\mathbb{P}}$ is empty. Let $\overline{\mathcal{T}}' = \overline{\mt}\setminus \overline{\mathbb{P}}$. If the uncontracted counterpart $\mt'$  has $\adm(\mt') \leq \zeta L_i$, we merge $\overline{\mathcal{T}}'$ with the last path added to $\overline{\mathbb{P}}$; otherwise, we add to $\overline{\mathbb{P}}$ the \emph{ minimal suffix}, say $\overline{\mp}'$, of $\overline{\mathcal{T}}'$ whose  uncontracted counterpart $\mp'$ has $\adm(\mp')\geq \zeta L_i$.  
	\end{itemize}	
   If any subpath, say $\overline{\mathcal{P}}_j \in \overline{\mathbb{P}}$ for some $j\in [1,t]$, is connected to a node in supercluster $\mx$ via an $\widetilde{\mst}_i$ edge $e$, then we add its uncontracted counterpart $\mathcal{P}_j$ and $e$ to $\mx$. Each of the remaining subpaths becomes a supercluster. (See Figure~\ref{fig:Step4-opt}.)
\end{itemize}
\end{itemize}


Note that in Step 4B, we cannot simply break the long path $\overline{\mt}$ into subpaths of augmented diameter at least $\zeta L_i$ (and at most $5\zeta L_i$) is because, for any subpath $\overline{\mp}$ of $\overline{\mt}$, $\adm(\mp) $ could be smaller than $\overline{\mp}$ by a super-constant factor; here $\mp$ is the uncontracted counterpart of $\overline{\mp}$.


%\noindent Note that constants chosen in Step 4 are somewhat arbitrary. The main point is to have subpaths of $\overline{\mathcal{T}}$ with an augmented diameter at least $5\zeta L_i$ so that we can show a lower bound $\zeta L_i$ on the agumented diameter of Step-4 superclusters (see Lemma~\ref{lm:Step4-Diameter-Lowerbound}).


\begin{lemma}\label{lm:Step4-Diam-Oracle}
		Every supercluster $\mx$ formed in Step 4 has: (a) $\varphi(\mx)\subseteq H_{\leq i}$, (b) $\zeta L_i \leq \adm(\mx)\leq 5\zeta L_i$  and (c) $|\mv(\mx)| = \Omega(\frac{1}{\epsilon})$ when $\epsilon \ll \frac{1}{g}$.
\end{lemma}
\begin{proof}
Let $\bar{\mx}$ be the subpath of a path $\overline{\mathcal{T}}$ formed in Step 4 that corresponds to $\mx$; $\mx$ is obtained from $\bar{\mx}$  by uncontracting supernode. Observe that $\mx$ is a subtree of $\widetilde{\mst}_i$ and hence $\varphi(\mx)\subseteq H_{\leq i-1} \subseteq H_{\leq i}$. Clearly $\adm(\mx)\geq \zeta L_i$ by construction. It remains to show the upper bound of $\adm(\mx)$.

Let $\overline{\mp} \in \overline{\mathbb{P}}$ be a subpath formed in Step 4B corresponding to $\mx$. Then by minimality of $\overline{\mp}$, $\adm(\mp)\leq  3\zeta L_i$ since each edge and node has weight at most $\zeta L_i$. If $\overline{\mp}$ is the last path added to $ \overline{\mathbb{P}}$, it could be merged with $\overline{\mt}'$. Since $\adm(\mt')\leq \zeta L_i$ and the $\widetilde{\mst}_i$ edge connecting $\mt'$ and $\mp$ has weight at most $\zeta L_i$, $\adm(\mp) \leq 5\zeta L_i$.

 The lower bound on the size of $\mv(\mx)$ follows from the same argument in Lemma~\ref{lm:Step2-Oracle-Diameter}.  \qed

% Additionally, $\adm(\mx)\leq \adm(\bar{\mx})$ by the way we assign weights to supernodes. Thus, $\adm(\mx)\leq 12\zeta L_i$. The lower bound on the size follows from the same argument in Lemma~\ref{lm:Step2-Oracle-Diameter}. \qed
\end{proof}

%We remark that proving lower bound on $\adm(\mx)$ is non-trivial; this is because for a supernode $\bar{\nu}$ in $\bar{\mx}$, $\adm(\md\cap \mathcal{T}_{\bar{\nu}})$ could be much smaller than $\omega(\bar{\nu})$. Here $\md$ is the diameter path of $\mx$. See Lemma~\ref{lm:Step4-Diameter-Lowerbound} for a detailed analysis.


After Step 4, all level-$i$ clusters are grouped into level-$(i+1)$ clusters. However, we have not done yet. In Step 5 below, we post-process superclusters. The goal is (i) to identify a subset of light nodes on which, together with heavy nodes, we construct a sparse spanner oracle, and (ii)  to show that, for each remaining light node, it is incident to only $O(1)$ edges on average.

\paragraph{Required definitions/preparations for Step 5.~} Let $\mx$ be a supercluster formed in previous steps.  Let $\doverline{\mathcal{K}_i}$ be a \emph{simple} cluster graph where $V(\doverline{\mathcal{K}_i})$ corresponds to superclusters, and there is an edge between two vertices if there is at least one level-$i$ edge between two corresponding superclusters. Note that there could be more than one edges between two candidate clusters, but we only keep (arbitrary) one of them in $\doverline{\mathcal{K}_i}$. We refer to vertices of $\doverline{\mathcal{K}_i}$  as \emph{meganodes}. For each meganode $\doverline{\nu}$, we denoted by $\mx_{\doverline{\nu}}$ the corresponding supercluster. 



We call a meganode $\doverline{\nu}$ a \emph{heavy} menganode if (a) $\mx_{\doverline{\nu}}$ contains at least $\frac{2g}{\zeta\epsilon}$ nodes -- in particular, $\doverline{\nu}$ is heavy if $\mx_{\doverline{\nu}}$ is formed in Step 1 -- or (b) it is incident to at least $\frac{2g}{\zeta\epsilon}$ edges in $\doverline{\mk_i}$. Otherwise, we call $\doverline{\nu}$ a \emph{light} meganode. Let $\doverline{\mathcal{V}}_{hv}$ be the set of heavy meganodes and $\doverline{\mathcal{V}}^+_{hv} = \doverline{\mathcal{V}}_{hv} \cup N_{\doverline{\mathcal{K}_i}}[\doverline{\mathcal{V}}_{hv}]$. It is possible that some heavy meganodes  --  those correspond to Step 1 superclusters -- are isolated vertices of $\mk_i$. 


Step 5 has three mini-steps, where in Step 5A, we will group all heavy meganodes and their neighbors into superclusters using the construction in Steps 1A and 1B. In Step 5B, we select a set of edges incident to light meganodes that do not have good stretch to $H_i$. In Step 5C, we add to $H_i$ edges of a sparse spanner oracle. Note that new superclusters are formed in Step 5A only.

\begin{wrapfigure}{r}{0.4\textwidth}
	\vspace{-25pt}
	\begin{center}
		\includegraphics[width=0.4\textwidth]{Step4-opt}
	\end{center}
	\caption{\footnotesize{A long path is broken into a set $\mathbb{P} = \{\overline{\mp}_1, \overline{\mp}_2,\overline{\mp}_3\}$ in Step 4B. $\overline{\mp}_2$ has an $\widetilde{\mst}_i$ edge to a supercluster $\mx$ formed in Steps 1-3 and hence it will be augmented to $\mx$ by construction.}}
	\vspace{-35pt}
	\label{fig:Step4-opt}
\end{wrapfigure}

\begin{itemize}
	\item \textbf{Step 5.~} This step has three mini steps.
	\begin{itemize}
		\item (Step 5A) We apply the same construction in Steps 1A and 1B to construct a collection of node-disjoint subtrees of $\doverline{\mathcal{K}_i}$, denoted by $\{\doverline{\mathcal{T}_1}, \ldots, \doverline{\mathcal{T}_k}\}$, where  each tree $\doverline{\mathcal{T}_j}$ has hop-diameter at most 6, and  $\cup_{j\in [k]}V(\doverline{\mathcal{T}_j}) = \doverline{\mathcal{V}}^+_{hv}$. For each tree  $\doverline{\mathcal{T}_j}$ with $j\in [k]$, we do the following: (i) make each tree $\doverline{\mathcal{T}_j}$ a supercluster by replacing each meganode by its corresponding supercluster and  (ii)  add level-$i$ edges of $\doverline{\mathcal{T}_j}$ to $H_i$.
		
		\item (Step 5B) For each supercluster $\mx$ corresponding to a light meganode in  $V(\doverline{\mathcal{H}_i})\setminus \doverline{\mathcal{V}}^+_{hv}$, we consider the set of level-$i$ edges incident to at least one node in $\mx$ in an arbitrary linear order. For each edge $e = (u,v)$ in the order, if $t\cdot w(e)\leq d_{H_{\leq i}}(u,v)$ we add $e$ to $H_i$.	
		
		\item (Step 5C) Let $\my$ be the set of nodes (of $\mg_i$) which are contained in superclusters formed in Step 5A.  For each node $\alpha\in \my$, we pick an arbitrary (real) vertex in $\varphi(\alpha)$; let $T$ be the set of picked vertices. We then update $H_i$ as:
		\begin{equation}\label{eq:add-oracle-refined}
		H_i\leftarrow H_i\cup E(\mathcal{O}_{G,t}(T,2L_i))
		\end{equation}
	\end{itemize}
	This completes our construction.
\end{itemize}


To complete the proof of Theorem~\ref{thm:cluster-opt-t2}, we need to (a) show that level-$(i+1)$ clusters satisfy all cluster properties (P1)-(P5),  (b) bound the stretch of edges in $E_i$ and (c) bound the weight of edges in $H_i$.  We prove (a) in Subsection~\ref{subsec:ClusterPropOracle}, (b) in Subsection~\ref{subsec:StretchOracle} and (c) in Subsection~\ref{subsec:HiWeightOracle}.


\subsubsection{Cluster Properties}\label{subsec:ClusterPropOracle}


In this section, we show that level-$(i+1)$ clusters satisfy all cluster properties. We say a supercluster $\mx$ is a Step-$j$ supercluster if it is formed in Step $j$ and become a level-$(i+1)$ cluster. First, we bound the augmented diameter of superclusters. 

\begin{lemma}\label{lm:Diameter-Up} $\varphi(\mx)\subseteq H_{\leq i}$ and $\zeta L_i \leq \adm(\mx) \leq  125L_i$ for any supercluster $\mx$. 
\end{lemma}
\begin{proof}
	If $\mx$ is formed in Steps 1-4, $\varphi(\mx)\subseteq H_{\leq i}$ by 
	Lemmas~\ref{lm:Step1-Diam-Oracle},~\ref{lm:Step2-Oracle-Diameter},~\ref{lm:Step3-Diam-Oracle}, and~\ref{lm:Step4-Diam-Oracle}. This also means that for any supercluster $\my$ corresponding to a meganode in Step 5, $\varphi(\my)\subseteq H_{\leq i}$. Since every edge of tree $\doverline{\mt}_j$ in Step 5A is added to $H_i$, the supercluster $\mx$ corresponding to  $\doverline{\mt}_j$ has $\varphi(\mx)\subseteq H_{\leq i}$. 
	
	It remains to bound $\adm(\mx)$. The lower bound follows directly from the construction.	 If $\mx$ is formed in Step 4B and becomes an independent supercluster,  then $\adm(\mx)~\leq~ 5\zeta L_i < L_i$ by Lemma~\ref{lm:Step4-Diam-Oracle}. Otherwise, excluding any augmentations to $\mx$ due to Step 4, Lemmas~\ref{lm:Step1-Diam-Oracle},~\ref{lm:Step2-Oracle-Diameter}, and~\ref{lm:Step3-Diam-Oracle} yield $\adm(\mx) \leq 13L_i$. We then may augment $\mx$ with trees of diameter at most $5\zeta L_i < L_i$ (Steps 4A and 4B). A crucial observation is that any augmented tree or subpath is connected by an $\widetilde{\mst}_i$ edge to a node that was clustered to $\mx$ at a previous step (Steps 1-3), hence all the augmented trees and subpaths are added to $\mx$ in a star-like way via $\widetilde{\mst}_i$ edges. If we denote the resulting supercluster by $\mx'$, then 
	\begin{equation*}
	\adm(\mx') \leq \adm(\mx) + 2\bar{w} + 2\cdot L_i \leq \adm(\mx) + 4L_i  \leq 17L_i, \end{equation*}
	
	
	If $\mx$ is formed in Step 5A, then by construction, it is formed by replacing each meganode $\doverline{\nu}$ of some subtree $\doverline{\mt}_j\subseteq \doverline{\mt}$ with the corresponding supercluster $\mx_{\doverline{\nu}}$ created in Steps 1-4. Since $\adm(\mx_{\doverline{\nu}})\leq 17 L_i$ and $\doverline{\mt}_j$ has hop diameter at most $6$, we have:
	\begin{equation*}
	\adm(\mx)\leq 6L_i + 7\cdot 17L_i = 125 L_i,
	\end{equation*}
	as desired.	\qed
\end{proof}

We are now ready to show that all cluster properties are satisfied. 

\begin{lemma} Level-$(i+1)$ clusters satisfy all cluster properties (P1)-P(5) with $g = 125$.
\end{lemma}
\begin{proof}
	Observe that property (P4) follows directly from the construction. Also by construction, superclusters are vertex-disjoint subgraphs of $\mg_i$. Thus, their source graphs, $\varphi(\mx)$ of each supercluster $\mx$, are vertex-disjoint.  This, with Lemma~\ref{lm:Diameter-Up}, implies property (P1). 	
	
	By Lemmas~\ref{lm:Step1-Diam-Oracle},~\ref{lm:Step2-Oracle-Diameter},~\ref{lm:Step3-Diam-Oracle} and~\ref{lm:Step4-Diam-Oracle}, each supercluster contains $\Omega(\frac{1}{\epsilon})$ nodes; this implies property (P2). Note that (P5) implies (P3) by Observation~\ref{obs:dm-vs-adm}, and (P5) follows directly from Lemma~\ref{lm:Diameter-Up}. \qed
\end{proof}

\subsubsection{Stretch}\label{subsec:StretchOracle}



In this section, we prove the stretch in $H_{\leq i}$ of edges in $E_i$ is at most $t(1+O(\epsilon))$. By setting $\epsilon \leftarrow \epsilon/c$ where $c$ is the constant behinds the big-O, we achieve a stretch of $t(1+\epsilon)$ by increasing the lightness by a   constant factor.  

%Let $e = (u,v)$ be an edge in $E_i$, let $\mbe$ be an edge of $\mathcal{K}_i$ corresponding to $e$ and let $\nu$ and $\mu$ be $\mbe$'s endpoints in $\mathcal{K}_i$. 

We observe that Claim~\ref{clm:e-not-inEi} remains true in this case, that we restate below.

\begin{claim}\label{clm:e-not-inEi-Oracle} If every edge in $\mathcal{E}_i$ has stretch $t\geq 1$ in $H_{\leq i}$, then every edge in $E_i$ has a stretch at most $t(1+O(\epsilon))$.
\end{claim}

Note that $\me_i$ is a subset of $E_i$ since we make $\mg_i(\mv_i,\me_i\cup\widetilde{\mst}_i,\omega)$ simple by removing parallel edges.

By Claim~\ref{clm:e-not-inEi-Oracle}, it remains to consider edges in $\mathcal{E}_i$. Let $e$ be such an edge. There are three cases: (1) $e \in \mathcal{B}_{close}$, (2) two endpoints of $e$ are nodes in $\mathcal{Y}$ in Step 5C,  or (3) $e$ is not selected in Step 5B. For Case (3), the stretch of $e$ is at most $t$ by construction. Thus, it remains to consider Case (1) and Case (2).

\begin{itemize}
	\item \text{Case 1:} $e \in \mb_{close}$. Let $\bar{\nu}$ and $\bar{\mu}$ be its endpoints.  Then  $\bar{\mi}(\bar{\nu})\cap \bar{\mi}(\bar{\mu}) \not=\emptyset$, hence there is a path $\overline{\mathcal{P}}$ of $\overline{\mathcal{F}}_2$ of weight at most $2L_i$ between $e$'s endpoint.  Since $\varphi(\overline{\mathcal{P}}[\bar{\nu},\bar{\mu}]) \subseteq H_{\leq i-1}$, it follows that there is a path of weight at most $2L_i$ between  $e$'s endpoints, say $u$ and $v$, in $H_{\leq i-1}$. Thus, for any $t\geq 2$, we have
	\begin{equation}
	d_{H_{\leq i}}(u,v) ~\leq~  2L_i \leq 2(1+\epsilon)\omega(e) < t(1+\epsilon)\omega(e) .
	\end{equation}
	
	\item \text{Case 2:} Two endpoints of $e$ are nodes in $\mathcal{Y}$ in Step 5C. Let $t_{\nu}, t_{\mu}$ be vertices chosen to $T$ in Step 5C.   By the triangle inequality, we have:
	\begin{equation}\label{eq:dist-terminals}
	\begin{split}
	d_G(t_{\mu}, t_{\mu}) &\leq \omega(e) + 2g\epsilon L_i \leq (1+2g\epsilon) L_i \leq 2L_i\\
	d_G(t_{\mu}, t_{\mu}) &\geq \omega(e) - 2g\epsilon L_i \geq (1-2g\epsilon) L_i \geq L_i/2
	\end{split}
	\end{equation}
	(Here we assume that $e$ is a shortest path between its endpoints; otherwise, we can remove all such edge $e$ at the outset of the algorithm in polynomial time.)  By Definition~\ref{def:oracle}, there is a path, say $P$, between $t_{\nu}, t_{\mu}$ in $\mathcal{O}_{G,t}(T, 2L_i)$ with $w(P)\leq t\cdot d_G(t_{\mu}, t_{\mu})$. This implies that:
	\begin{equation}\label{eq:stretch-heavy}
	\begin{split}
	d_{H_{\leq i}}(u,v) &\leq d_{\varphi(\mu)}(u,t_{\mu}) + d_{\mathcal{O}_{G,t}(T, 2L_i)}(t_{\mu}, t_{\nu}) + d_{\varphi(\nu)}(t_{\nu},v)\\
	&\leq g\epsilon L_i + t d_G(t_{\mu}, t_{\nu}) + g\epsilon L_i \\
	&\leq g\epsilon L_i + t \left(\omega(e) + 2g\epsilon L_i \right) + g\epsilon L_i \\
	&\leq t \omega(e) + t 3g\epsilon L_i \leq t(1 + 6g\epsilon) \omega(e).
	\end{split}
	\end{equation}
	Thus, the stretch of  $e$ in any case is $t(1+O(\epsilon))$. \qed
\end{itemize}

\subsubsection{Bounding $w(H_i)$}\label{subsec:HiWeightOracle}


We now show that the total weight of edges added to $H_i$ is bounded by local potential reduction (see Equation~\eqref{eq:LocalPotential} and Lemma~\ref{lm:GlobalToLocalPotential}).  First, we observe that:

\begin{claim}\label{clm:ADM-vs-Size}
	For any path $\mp$ of $\mg_i(\mv_i,\me_i\cup \widetilde{\mst}_i,\omega)$, $\adm(\mp) = \Omega(|\mv(\mx)| \epsilon L_i)$.
\end{claim}
\begin{proof}
	By definition of augmented diameter,
	\begin{equation*}
	\begin{split}
	\adm(\mp) &= \sum_{\alpha \in \mv(\mp)}\omega(\alpha) + \sum_{e\in \me(\mp)}\omega(e)  \geq \sum_{\alpha \in \mv(\mp)}\omega(\alpha) \stackrel{\mbox{\tiny{P(5)}}}{\geq}  \sum_{\alpha \in \mv(\mp)}\zeta L_{i-1}= \Omega(|\mv(\mp)| \epsilon L_i),
	\end{split}
	\end{equation*}
as desired.
\qed
\end{proof}
For each $j \in [1,5]$, let $\mathbb{X}_j$ be the set of superclusters that are initially formed in Step $j$ and could possibly be augmented in Step 4A. (Clearly, superclusters in Step 5A are not augmented in Step 4A.) We start with superclusters formed in Step 1 and 5.

\begin{lemma}\label{lm:Step15WeightOracle}
	Let $\mx \in \mathbb{X}_1 \cup \mathbb{X}_5$ be a supercluster formed in  Steps 1 or 5, then:
	\begin{equation*}
	\Delta^i_{L}(\mx) = \Omega(|\mv(\mx)|\epsilon L_i)  
	\end{equation*}
\end{lemma}
\begin{proof} Let $\mx \in \mathbb{X}_1$ be a supercluster formed in Step 1 or 5.	By construction, $\mx$ has at least $\frac{2g}{\zeta \epsilon}$ nodes. Thus,  by definition of local potential reduction (Equation~\eqref{eq:LocalPotential}), we have:
	\begin{equation}
	\begin{split}
	\Delta^i_L(\mx) &\geq \sum_{\alpha \in \mx}w(\alpha)  - \adm(\mx) \stackrel{(P5)}{\geq} \sum_{\alpha \in \mx}\zeta L_{i-1} - gL_i  = \frac{|\mv(\mx)| \zeta L_{i-1}}{2} + \underbrace{(\frac{|\mv(\mx)| \zeta L_{i-1}}{2} - gL_i)}_{\geq 0 \mbox{ since }|\mv(\mx)|\geq (2g)/(\zeta \epsilon)}\\
	&\geq  \frac{|\mv(\mx)| \zeta L_{i-1}}{2}  = \Omega(|\mv(\mx)|\epsilon L_{i}),
	\end{split}
	\end{equation}
	as desired. \qed 
\end{proof}


We now bound the local potential reduction of superclusters in Step 2. To show that Step-2 superclusters have a large potential reduction, we rely on the fact that they have three internally vertex disjoint paths of augmented weight proportional to the augmented diameter of the supercluster-- Item (4) in Lemma~\ref{lm:tree-clustering}.

Let $\mz$ be a subgraph of $\mg_i(\mv_i,\me_i\cup \widetilde{\mst}_i,\omega)$. We define the potential of $\mz$ by:
\begin{equation}\label{eq:mz}
\Phi(\mz) = \sum_{\alpha \in \mv(\mz)}\omega(\alpha) + \sum_{e \in \widetilde{\mst}_i\cap \me(\mz)} \omega(e)
\end{equation}
Since $\omega(e)\leq \omega(\alpha) \leq g\epsilon L_i$ for every $e \in \widetilde{\mst}_i\cap \me(\mz)$, we have:
\begin{equation}\label{eq:Potential-vs-Size}
\Phi(\mz) = \Omega(|\mv(\mz)|\epsilon L_i)
\end{equation}


\begin{wrapfigure}{r}{0.3\textwidth}
	\vspace{-25pt}
	\begin{center}
		\includegraphics[width=0.3\textwidth]{Step2-opt-potential}
	\end{center}
	\caption{\footnotesize{Diameter path $\md$ is marked by the dashed purple curve. Subtrees enclosed by dash red curves are augmented to $\mx$ in Step 4.}}
	\vspace{-10pt}
	\label{fig:Step2-opt-potential}
\end{wrapfigure}


\begin{lemma}\label{lm:Step2ClusterOracle}
	Let $\mx \in \mathbb{X}_2 $ be a supercluster formed in  Step 2, then:
	\begin{equation*}
	\Delta^i_{L}(\mx) = \Omega(|\mv(\mx)|\epsilon L_i)  
	\end{equation*}
\end{lemma}
\begin{proof} 	Let $\mathcal{T}\subseteq \mathcal{F}_1$ be the part of $\mx$ formed in Step 2;  $\mx$ is obtained from $\mathcal{T}$ by (possible) augmentation in Step 4A. By Item (2) of Lemma~\ref{lm:tree-clustering}, there is a $\mathcal{T}$-branching node $\nu$ and three paths $\mathcal{P}_1,\mathcal{P}_2,\mathcal{P}_3$ sharing $\nu$ as the same endpoints such that $\adm(\mathcal{P}_j\setminus \{\nu\}) = \Omega(\adm(\mathcal{T}))) = \Omega(\zeta L_i)$ for $j \in [3]$.
	
	For each tree $\overline{\ma}$ in Step 4A that is augmented to $\mt$, by uncontracting supernodes in $\overline{\ma}$, we obtain a subtree $\ma$ of $\mathcal{F}_1$ of augmented diameter at most $12\zeta L_i$. Thus, $\mx$ remains to be a subtree of $\mathcal{F}_1$ after the augmentation in Step 4A since each tree is augmented to $\mathcal{T}$ via $\widetilde{\mst}_i$ edges. 
	
	Let $\mathcal{D}\subseteq \mathcal{F}_1$ be the diameter path of $\mx$. Then by definition of augmented diameter, 
	\begin{equation*}
	\adm(\mx)  = \sum_{\alpha \in \md}\omega(\alpha) + \sum_{\tilde{e \in \me(\md) }} \omega(e)
	\end{equation*}
	
	Let $\my = \mx\setminus \md$. Since $\nu$ is $\mathcal{T}$-branching, there must exist $j \in [3]$ such that $\md\cap \mathcal{P}_j \subseteq \{\nu\}$. Since $\omega(\nu)\leq g L_{i-1} = g\epsilon L_i$ by property (P5) and the $\widetilde{\mst}_i$ incident to $\nu$ in $\mp_j$ has length at most $L_{i-1} = \epsilon L_i$, we have:
	\begin{equation*}
	\adm(\mathcal{P}_j\setminus \{\nu\}) \geq \adm(\mp_j) - (g+1)\epsilon L_i = \Omega(\zeta L_i) = \Omega(L_i)
	\end{equation*}
	when $\epsilon \ll \frac{1}{g}$. Thus, $\Phi(\my)\geq \adm(\mathcal{P}_j) = \Omega(L_i)$, and hence:
	\begin{equation}\label{eq:PhiY-sizeD}
	\Phi(\my)/2 = \Omega(L_i) = \Omega(\adm(\md)) = \Omega(|\mv(\md)|\epsilon L_i) \qquad \mbox{by Claim~\ref{clm:ADM-vs-Size}}
	\end{equation}
	In Equation~\eqref{eq:PhiY-sizeD}, we use the fact that $\adm(\md) \leq gL_i =  O(L_i)$ by property (P5). We have:
	\begin{equation*}
	\begin{split}
	\Delta^i_L(\mx) &=  \sum_{\alpha \in \md}\omega(\alpha) + \sum_{\tilde{e} \in \me(\mx)} \omega(e) - \adm(\mx)\\
	&\geq \Phi(\my)  =  \frac{\Phi(\my)}{2} +\Omega(|\mv(\md)|\epsilon L_i) \qquad \mbox{by Equation~\eqref{eq:PhiY-sizeD} }\\
	&\geq  \frac{|\my| \zeta L_{i-1}}{2} +\Omega(|\mv(\md)|\epsilon L_i)\\
	&= \Omega(|\my| \epsilon L_i) +\Omega(|\mv(\md)|\epsilon L_i) = \Omega(|\mv(\mx)|\epsilon L_i),
	\end{split}
	\end{equation*} 
	as desired.\qed
\end{proof}

When comparing potential reduction of Step-2 superclusters in Lemma~\ref{lm:Step2ClusterOracle} and Lemma~\ref{lm:Step2Cluster}, the amount of potential in this construction is about $\frac{1}{\epsilon}$ times bigger the amount of potential in the previous construction. This is one of the key properties to reduce the dependency on $\epsilon$ of lightness to linear in $\frac{1}{\epsilon}$.

\noindent We now turn to Step-3 superclusters. Similar to Lemma~\ref{lm:Step3Cluster}, we can show large potential reduction of superclusters in this step.

 \begin{wrapfigure}{r}{0.4\textwidth}
	\vspace{-35pt}
	\begin{center}
		\includegraphics[width=0.4\textwidth]{Step3-opt-dm}
	\end{center}
	\caption{\footnotesize{(a) $\md$ does not contain $e$ and (b) $\md$ contains $e$. Nodes enclosed by dashed red curves are added to $\mx$ in Step 4.}}
	\vspace{-10pt}
	\label{fig:Step3-opt-dm}
\end{wrapfigure}

\begin{lemma}\label{lm:Step3ClusterOracle}
	Let $\mx \in \mathbb{X}_3 $ be a supercluster formed in  Step 3, then:
	\begin{equation*}
	\Delta^i_{L}(\mx) = \Omega(|\mv(\mx)|\epsilon L_i)  
	\end{equation*}
\end{lemma}
\begin{proof} Let $\md$ be a diameter path of $\mx$, and $\my = \mx \setminus \mv(\md)$.	Let $\overline{P}$ be a path of $\overline{\mf}_2$ where $\overline{\mf}_2$ is the forest formed at the beginning of Step 3. We observe that:
\begin{observation}\label{obs:path-to-forest} Let $\mt$ be the tree obtained from $\overline{\mp}$ by uncontracting supernodes. Then $\Phi(\mt)\geq \adm(\overline{\mp})$.
\end{observation}	
\begin{proof}
	For each node $\bar{\nu}\in \overline{\mp}$, the corresponding tree $\mt_{\bar{\nu}}$ obtained by uncontracting $\bar{\nu}$ has $\Phi(\mt_{\bar{\nu}})\geq \adm(\mt_{\bar{\nu}}) = \omega(\bar{\nu})$. Thus, 
	
	\begin{equation*}
	\begin{split}
		\Phi(\mt) \geq \sum_{\bar{\nu}\in \mv(\overline{\mp})}\Phi(\mt_{\bar{\nu}}) + \sum_{e\in E(\overline{\mp})} \omega(e)
		 \geq   \sum_{\bar{\nu}\in \mv(\overline{\mp})}\omega(\bar\nu) + \sum_{e\in E(\overline{\mp})} \omega(e) = \adm(\overline{\mp}),
	\end{split}
	\end{equation*}
as desired. \qed
\end{proof}
	
	 Let $\bar{\mi}(\bar\nu)$ and $\bar\mi(\bar\mu)$ be two intervals  in the construction on Step 3 that are connected by an edge $\mbe = (\nu,\mu)$.
	 
	
	\begin{claim}\label{clm:PotentialY-boundOracle} $\Phi(\my)=  \frac{5L_{i} }{4}+ \Omega(|\mv(\my)|\epsilon L_i)$.
	\end{claim}
	\begin{proof} We consider two cases:
		\begin{itemize}
			\item \emph{Case 1: $\md$ does not contain the edge $(\nu,\mu)$.} See Figure~\ref{fig:Step3-opt-dm}(a). In this case, $\md \subseteq  \widetilde{\mst}_i$, and  that $\bar\mi(\bar\nu)\cap\md =\emptyset$ or $\bar\mi(\bar\mu)\cap \md = \emptyset$ since $\bar\mi(\bar\nu)$ and $\bar\mi(\bar\mu)$ are connected only by $e$. We assume w.l.o.g. that  $\bar\mi(\bar\nu)\cap\md =\emptyset$.  Then, by Observation~\ref{obs:path-to-forest} and Claim~\ref{clm:Interval-node-unified}, it holds that:
			\begin{equation*}
			\Phi(\my)\geq \adm(\overline{\mathcal{I}}(\bar\nu)) \geq (2-(3\zeta+2)\epsilon) L_i\geq \frac{5L_i}{3}
			\end{equation*}
		    when $\epsilon \ll \zeta$.
		    
			\item  \emph{Case 2: $D$ contains the edge $(\nu,\mu)$.} See Figure~\ref{fig:Step3-diam}(b). In this case at least two sub-intervals, say $\bar\mi_1,\bar\mi_2$,  of four intervals $\{\bar\mi(\bar\nu)\setminus \bar\nu, \bar{\mi}(\bar\mu)\setminus \bar\mu\}$ are disjoint from $\md$. By minimality of  $\bar\mi(\bar\nu)$ and $\bar\mi(\bar\mu)$, $\adm(\bar\mi_j)\geq L_i - 2(\zeta L_i + \epsilon L_i) ~=~ L_i - 2(\zeta+\epsilon) L_i$, where $g\epsilon L_i$  is the upper bound on the node weight and $\epsilon L_i$ is the upper bound on the weight of $\widetilde{\mst}_i$ edge.   By Observation~\ref{obs:path-to-forest}, it holds that:
			\begin{equation*}
			\Phi(\my)\geq \Phi(\mb)\geq \adm(\overline{\mi}_1) + \adm(\overline{\mi}_2) 	\geq (2- 4(\zeta + \epsilon) L_i \geq \frac{5L_i}{3}
			\end{equation*}
			when $\epsilon \ll \zeta$.
		\end{itemize}	
		Thus, in both cases, $\Phi(\my) \geq \frac{5L_i}{3}$. This implies:
		\begin{equation*}
		\begin{split}
		\Phi(\my) &= \frac{3 \Phi(\my)}{4}  + \frac{\Phi(\my)}{4} \geq \frac{3}{4}\frac{5}{3} L_i + \frac{\Phi(\my)}{4} \\
		&\geq \frac{5 L_i}{4} +  \frac{\Phi(\my)}{4}  = \frac{5 L_i}{4}  +  \Omega(|\mv(\my)|\epsilon L_i) \qquad \mbox{by Equation~\eqref{eq:Potential-vs-Size}},		
		\end{split}
		\end{equation*} 
		as desired \qed. 
	\end{proof}


We now bound $\Delta^i_{L}(\mx)$. By definition of local potential reduction, we have:
\begin{equation*}
\begin{split}
	\Delta_{L}^i(\mx)  &= \Phi(\md) + \Phi(\my) - \adm(\mx)\\
&= \Phi(\my) - \omega(\mbe) \geq  \frac{L_i}{4}  +  \Omega(|\mv(\my)|\epsilon L_i) \quad \mbox{by Claim~\ref{clm:PotentialY-boundOracle}}\\
&= \Omega(|\mv(\md)|\epsilon L_i) +  \Omega(|\mv(\my)|\epsilon L_i) \quad \mbox{by Claim~\ref{clm:ADM-vs-Size}}\\
&= \Omega(|\mv(\mx)|\epsilon L_i), 
\end{split}
\end{equation*}
as desired. \qed
	\end{proof}


We are now ready to bound $w(H_i)$. Recall that by construction, we only add edges to $H_i$ in Step 1, Step 3, and Step 5. 

\begin{lemma}\label{lm:H5A} Let $H^{\leq 5A}_i$ be edges added to $H_i$ in  Steps 1, 3 and 5A. Then $w(H^{\leq 5A}_i) = O(\frac{1}{\epsilon}) \Delta^i_{L}$.
\end{lemma}
\begin{proof}
Observe by construction that for every supercluster $\mx$ formed in Steps 1, 3 or 5A, the number of level-$i$ edges added to $H_i$ during the construction of $\mx$ is at most $|\mv(\mx)|$ since $\mx$ is a tree; this implies:
\begin{equation*}
w(H^{\leq 5A}_i)  \leq \sum_{\mx \in \mathbb{X}_1\cup \mathbb{X}_3\cup \mathbb{X}_5} |\mv(\mx)| L_i
\end{equation*}
By Lemma~\ref{lm:Step15WeightOracle} and Lemma~\ref{lm:Step3ClusterOracle}, $|\mv(\mx)| L_i = O(\frac{1}{\epsilon})\Delta^i_{L}(\mx)$. Thus, it holds that:
\begin{equation*}
w(H^{\leq 5A}_i)   = O(\frac{1}{\epsilon}) \sum_{\mx \in \mathbb{X}_1\cup \mathbb{X}_3\cup \mathbb{X}_5} \Delta^i_{L}(\mx) = O(\frac{1}{\epsilon}) \Delta^i_{L}
\end{equation*}
by Lemma~\ref{lm:GlobalToLocalPotential}.\qed
\end{proof}

It remains to bound the total weight of edges added to $H_i$ in Steps 5B and 5C. We start with edges added in Step 5C.

\begin{lemma}\label{lm:H5C}
	Let $H_i^{5C}$ be the set of edges added to $H_i$ in Step 5C. Then $w(H_i^{5C}) = O(\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon})\Delta^i_{L}$.
\end{lemma}
\begin{proof} Recall that all nodes in the set $\my$ in the construction of Step 5C are in Step-5A supercluters. Note that  $w(E(\mathcal{O}_{G,t}(T,2L_i))) = O(\wsp_{\mathcal{O}_{G,t}} |T| L_i)$ by Definition~\ref{def:oracle}, and that $|T| = \sum_{\mx\in \mathbb{X}_5}|\mv(\mx)|$. Thus, with Lemma~\ref{lm:Step15WeightOracle}, we have:
	\begin{equation*}
	\begin{split}
		w(H_i^{5C}) &= w(E(\mathcal{O}_{G,t}(T,2L_i)))   = O(\wsp_{\mathcal{O}_{G,t}})  \sum_{\mx\in \mathbb{X}_5}|\mv(\mx)| L_i\\
		 &= O(\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon}) \sum_{\mx\in \mathbb{X}_5} \Delta^i_{L}(\mx) \leq O(\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon}) \Delta^i_{L},
	\end{split}
\end{equation*}
as desired. \qed	
\end{proof}


We now focus on bounding edges of $\me_{i}$ added to $H_i$ in Step 5B.  Let $\mx$ a supercluster corresponding to light meganode. By definition of light meganodes, there are $O(\frac{1}{\epsilon})$ edges incident to $\mx$ in $\doverline{\mk}_i$. We can show that $\mx$ has $\Omega(\frac{1}{\epsilon})$ nodes, and hence, on average, each node is incident to $O(1)$ edges. One may conclude that the total weight of these edges is only at most $O(\frac{1}{\epsilon})$ times potential reduction of $\mx$. However, there remain two issues: (1) between two superclusters, there could be more than one edge; we deliberately remove all but one in the construction of $\doverline{\mk}_i$, and (2) there could be many edges between two nodes in the same supercluster $\mx$. Our key insight is that, between any two superclusters, the construction in Step 5C only keeps at most $O(1)$ level-$i$ edges; the same holds for level-$i$ edges between nodes in the same supercluster. 


\begin{lemma}\label{lm:key-incident}
	Let $\mx$ be a light supercluster corresponding to a meganode in the construction of Step 5C. Then, the number of level-$i$ edges added to $H_i$ with \emph{both endpoints} in $\mx$ is $O(1)$. Similarly,  for any supercluster $\mx' \not = \mx$, there are at most $O(1)$ level-$i$ edges added to $H_i$ between $\mx'$ and $\mx$.
\end{lemma}
\begin{proof} When we say two light superclusters are adjacent in $\doverline{\mathcal{K}_i}$, we mean their corresponding meganodes are adjacent in $\doverline{\mathcal{K}_i}$.  First, we observe that any supercluster adjacent to $\mx$ in $\doverline{\mathcal{K}_i}$ is light since every neighbor of a heavy meganode is grouped in Step 5A. This implies that $\mx$ is not formed in Step 1  by the definition of a heavy meganode.
	
	We consider the following decomposition $\mathbb{D}_\mx$ of $\mx$ into \emph{small superclusters}:
	\begin{itemize}
		\item  If $\mx$ is formed in Steps 2 or 4, then $\mathbb{D}_\mx = \{\mx\}$.
		\item  Otherwise, $\mx$ is formed in Step 3. By construction, it has  two intervals $\bar\mi_{\bnu}$ and $ \bar{\mathcal{I}}_{\bmu}$ connected by a level-$i$ edge $(\bnu,\bmu)$, and a set of trees $\mathbb{U}= \{\overline{\mathcal{T}_1}, \overline{\mathcal{T}_2}, \ldots, \overline{\mathcal{T}_p}\}$  each of augmented diameter at most $\zeta L_i$ which are connected to nodes in $\bar{\mathcal{I}}_{\bnu}\cup \bar{\mathcal{I}}_{\bmu}$ via $\widetilde{\mst}_i$ edges due to the augmentation in Step 4. 

		We greedily partition each interval, say $\bar{\mathcal{I}}_{\bnu}$, into node-disjoint, subintervals of augmented diameter at most $3\zeta L_i$ and at least $\zeta L_i$; let $\{\bar{\ma}_1, \ldots, \bar{\ma}_{q}\}$ be the set of all the subintervals. Let $\ma_j$, $j\in [q]$, be obtained from $\bar{\ma}_j$ by uncontracting non-trivial supernodes. 
		We extend each $\mathcal{A}_j$ to include all trees in $\mathbb{U}$ that are connected to nodes in $\mathcal{A}_j$ by $\widetilde{\mst}_i$ edges. We denote the extension of $\mathcal{A}_j$ by $\mathcal{A}_j^{+}$. We then add all trees in  $\{\mathcal{A}_1^{+}, \ldots, \mathcal{A}_q^{+}\}$ to $\mathbb{D}_\mx$. (See Figure~\ref{fig:Iv-partition}.)
	\end{itemize}

\begin{wrapfigure}{r}{0.4\textwidth}
	\vspace{-35pt}
	\begin{center}
		\includegraphics[width=0.4\textwidth]{Iv-partition}
	\end{center}
	\caption{\footnotesize{$\overline{\ma}_j$ is inclosed by green-shaded region, and $\ma_j^+$ is enclosed by a dashed blue curve for every $j\in [1,4]$.}}
	\vspace{-10pt}
	\label{fig:Iv-partition}
\end{wrapfigure}
	\begin{claim}\label{clm:Size-DC}$\mathbb{D}_\mx$ has the following properties:
		\begin{enumerate}
			\item $|\mathbb{D}_\mx| = O(1)$
			\item For any $\ma \in\mathbb{D}_\mx$,  $\adm(\ma) \leq 29\zeta L_i$ when $\epsilon < \zeta$.
			\item  There is at most one level-$i$ edge, if any, in $H_i$ connecting two different small superclusters in $\mathbb{D}_\mx$.
		\end{enumerate}
	\end{claim}
	\begin{proof}
		By Claim~\ref{clm:Interval-node-unified}, $\bar{\mathcal{I}}_{\nu}$ has augmented diameter at most $2L_i$. This implies
		\begin{equation}
		|\mathbb{D}_\mx| \leq 2\times\frac{2L_i}{\zeta L_i} = O(1)
		\end{equation}
		
		Since the extension of each $\ma_j$ is via $\widetilde{\mst}_i$ edges in a star-like way, $\adm(\mathcal{A}_j^{+})~\leq~ \adm(\mathcal{A}_j) + 2\bar{w} + 2\cdot \zeta L_i \leq 5\zeta L_i + 2\epsilon L_i \leq 7\zeta L_i$.
		
		For the third item, assume that  in Step 5B the algorithm takes to $H_i$ two edges $(u,v), (u',v')$ between two small superclusters $\ma,\ma'$ in $\mathbb{D}_\mx$ where $\{u,u'\}\subseteq \varphi(\ma),  \{v,v'\}\subseteq \varphi(\ma')$.~W.l.o.g, we assume that $(u',v')$ is considered before $(u,v)$. Let $P_{uv}$ be a shortest path between $u$ and $v$ before $(u,v)$ is added.  Then, by the triangle inequality,
		\begin{equation}
		\begin{split}
		w(P_{uv})&\leq w(u',v') + \adm(\ma) + \adm(\ma') \leq  w(u',v') + 14\zeta L_i \\
		w(u',v')&\leq w(u,v) + \adm(\ma) + \adm(\ma') \leq  w(u,v) + 14\zeta L_i
		\end{split}
		\end{equation}
		Thus  $w(P_{uv}) \leq w(u,v) + 28\zeta L_i ~\stackrel{w(u,v)\geq L_i/2}{\leq}~ (1+56\zeta) w(u,v)  ~<~ t\cdot w(u,v)$ since $\zeta = \frac{1}{250}$ and $t\geq 2$. Thus, edge $(u,v)$ will not be added to $H_i$ in Step 5B;  a contradiction.\qed
	\end{proof}
	Items (1) and (3) in Claim~\ref{clm:Size-DC} immediately imply the first claim in Lemma~\ref{lm:key-incident}.  For the second claim, observe that for any two small superclusters in $\mathbb{D}_\mx$ and $\mathbb{D}_{\mx'}$, by the same proof of Item (3) in Claim~\ref{clm:Size-DC}, there is at most one level-$i$ edge in $H_i$ between them. Thus, by Item (1), there are at most $O(1)$ level-$i$ edges connecting $\mx$ and $\mx'$.
	\qed
\end{proof}

A simple corollary of Lemma~\ref{lm:key-incident} is the following.

\begin{corollary}\label{cor:deg-C-5B}
	For any light supercluster $\mx$ considered in  Step 5B, there are $O(\frac{1}{\epsilon})$ level-$i$ edges incident to nodes in $\mx$ that are added to $H_i$ in Step 5B.
\end{corollary}
\begin{proof}
	By construction, $\mx$ is a light supercluster: it has at most $\frac{2g}{\zeta\epsilon} = O(\frac{1}{\epsilon})$ neighbors in $\doverline{\mathcal{K}_i}$.  For each neighbor $\mx'$ of $\mx$, by Lemma~\ref{lm:key-incident}, there are $O(1)$ level-$i$ edges between $\mx$ and $\mx'$ added $H_i$. Thus, there are $O(\frac{1}{\epsilon})$ level-$i$ edges in $H_i$ such that each has exactly one endpoint in $\mx$. Also by Lemma~\ref{lm:key-incident}, there are at most $O(1)$ level-$i$ edges with both endpoints in $\mx$; this implies the corollary.\qed
\end{proof}

We are now ready to bound the total weight of edges added to $H_i$ in Step 5C.

	\begin{figure}[hbt]
	\centering
	%\vspace{-20pt}
	\includegraphics[scale = 0.9]{longpath-opt}
	\caption{\footnotesize{A set of paths $\overline{\mathbb{P}} = \{\overline{\mp}_1,\ldots,\overline{\mp}_9\}$ broken from a long path $\overline{\mp}$. Subpath $\overline{\mp}_5$ is augmented to a supercluster $\my$ formed in Steps 1-3. Red paths of $\overline{\mp}$ are enclosed in dashed red curves; other paths are blue paths.   Red edges are level-$i$ edges taken to $H_i$; there is no red edge between any two blue paths. Non-trivial supernodes are triangular shaded regions. }}
	\label{fig:longpath-opt}
\end{figure}

\begin{lemma}\label{lm:H5B} Let $H^{5B}_{i}$ be the set of edges added to $H_i$ in Step 5B. If there is at least one supercluster formed in Steps 1-3, then $w(H^{5B}_i) = O(\frac{1}{\epsilon}) \Delta^i_{L}$.
\end{lemma}
\begin{proof}	Let $\mx$ be a light supercluster considered in Step 5B. By the construction in Step 5A and definition of heavy superclusters, $\mx$ must be formed in Steps 2-4. Let $H^{5B}_i(\mx)$ be the set of edges in $H^{5B}_i$ that are incident to nodes in $\mx$.	We consider two cases:
	
\noindent \textbf{Case 1.~} $\mx$ is formed in Steps 2 or 3. Then by Corollary~\ref{cor:deg-C-5B}, $w(H^{5B}_i(\mx)) = O(\frac{L_i}{\epsilon}) = O(|\mv(\mx)|L_i)$ since $\mx$ has at least $\Omega(\frac{1}{\epsilon})$ nodes by property (P2). By Lemmas~\ref{lm:Step2ClusterOracle} and~\ref{lm:Step3ClusterOracle}, we have:
	\begin{equation}\label{eq:H5B1}
	\sum_{\mx\in \mathbb{X}_2\cup \mathbb{X}_3} w(H^{5B}_i(\mx)) = O(\frac{1}{\epsilon}) \sum_{\mx\in \mathbb{X}_2\cup \mathbb{X}_3} \Delta^i_{L}(\mx) \leq  O(\frac{1}{\epsilon}) \Delta^i_{L}
	\end{equation}


\noindent \textbf{Case 2.~} $\mx$  is formed in Step 4; in particular, $\mx$ is formed in Step 4C. Then $\mx$ is the uncontracted counterpart of a subpath $\overline{\mp}_a$ of a long path, say $\overline{\mathcal{P}}$, in $\overline{\mathcal{F}_3}$. That is, $\mx$ is obtained from $\overline{\mp}_a$ by uncontracting non-trivial supernodes. (See Figure~\ref{fig:longpath-opt}.) By construction in Step 4B, $\overline{\mp}$ is broken into a set of subpaths $\overline{\mathbb{P}} = \{\overline{\mp}_1, \ldots, \overline{\mp}_t\}$; $\mp_j$ is the uncontracted counterpart of $\overline{\mp}_j$.

Since $\widetilde{\mst}_i$ is a spanning tree of $\mg_i$ by  Lemma~\ref{lm:spanning-Gi}, there must be an $\widetilde{\mst}_i$ edge connecting a node in $\mp$ to a node clustered in Steps 1-3. Thus, by construction in Step 4B, there must a subpath $\overline{\mp}_j \in \overline{\mathbb{P}}$ for some $j \in [1,t]$ that is added to a supercluster, say $\my$, formed in Steps 1-3  ($\my$ may be grouped to a bigger supercluster in Step 5A). Note that $\my$ exists by the assumption that there is at least one supercluster formed in Steps 1-3. 

Recall that in Step 3, nodes in augmented distance at most $L_i$ from at least one of the endpoints of $\overline{\mp}$ are colored red, and other nodes are colored blue. We call a path $\overline{\mp}_b \in \overline{\mathbb{P}}$, $b\in [1,t]$, a \emph{red path} if it contains \emph{at least one red node}; otherwise, we call $\overline{\mp}_b$ a blue path.

We have two claims:
\begin{itemize}
	\item \textit{Claim A: the number of red paths in $\overline{\mathbb{P}}$ is $O(1)$}.   Observe that each red path $\overline{\mp}_b \in \overline{\mathbb{P}}$ has $\adm(\overline{\mp}_b)\geq \adm(\mp_b) \geq \zeta L_i$. Since red nodes are in the prefix and suffix of $\overline{\mp}$ of augmented diameter at most $L_i$ each, the number of red paths is at most $\frac{2L_i}{\zeta L_i} = O(1)$ as claimed.
	\item \textit{Claim B: there is no level-$i$ edge added $H_i$  between two blue paths}. Suppose there is such an edge, say $\mbe$, then either $\mbe \in \mb_{far}$ or $\mbe \in \mb_{close}$ (see Equation~\eqref{eq:Bfar-Bclose}). $\mbe$ cannot be in $\mb_{far}$ since such an edge will be handled in Step 3, and $\mbe$ cannot be in $\mb_{close}$ since we discard every in $\mb_{close}$ in Step 4. Thus, there is no such edge $\mbe$. 
\end{itemize}

%$\adm(\mx)\leq 5\zeta L_i$ by Lemma~\ref{lm:Step4-Diam-Oracle}. 
 We consider two subcases:

\begin{itemize}
	\item 	 \emph{Case 2A: $\overline{P}_a$ is a red path of $\overline{\mathbb{P}}$.~}  By Lemmas~\ref{lm:Step15WeightOracle},~\ref{lm:Step2ClusterOracle}, and~\ref{lm:Step3ClusterOracle}, by redistributing the potential reduction of the supercluster containing $\my$ to its nodes evenly, each node gets $\Omega(\epsilon L_i)$ unit.  
	
	Recall $\mp_j$ is the uncontracted counterpart of $\overline{\mp}_j$ (obtained by uncontracting non-trivial supernodes). ($\overline{\mp}_j$ is $\overline{\mp}_5$ in Figure~\ref{fig:longpath-opt}.) Then, $\Phi(\mp_j)\geq \adm(\mp_j) \geq \zeta L_i$ by Lemma~\ref{lm:Step4-Diam-Oracle}. Since every edge has weight at most $L_{i-1} =\epsilon L_i$ and every node has weight at most $gL_{i-1} = g\epsilon L_i$ by property (P5), we have:
	\begin{equation*}
	|\mv(\mp_j)| \geq \frac{\Phi(\mp_j)}{g\epsilon L_i} \geq \frac{\zeta}{\epsilon g} = \Omega(\frac{1}{\epsilon})
	\end{equation*}
	
	Thus, nodes in $\mp_j$ get at least $\Delta\Phi(\mp_j) \stackrel{\mbox{\tiny{def.}}}{=} |\mv(\mt_j)|\Omega(\epsilon L_i) ~=~ \Omega(L_i)$ unit of potential distributed from $\my$.	We use the potential of $\mp_j$ to bound the total weight of edges in $H_i$ incident to nodes in \emph{all red paths} in $\overline{\mathbb{P}}$; there are $O(\frac{1}{\epsilon})$ such edges by Claim A and Corollary~\ref{cor:deg-C-5B}. The total weight of these edges is $O(\frac{1}{\epsilon})\Delta\Phi(\mp_j)$. This implies that the total weight of edges incident to superclusters considered in this case is:
	\begin{equation}\label{eq:H5B3}
	O(\frac{1}{\epsilon})\left(\sum_{\my \in \mathbb{X}_1 \cup \mathbb{X}_2 \cup \mathbb{X}_3\cup \mathbb{X}_5}\Delta^i_{L}(\my)\right) = O(\frac{1}{\epsilon})\Delta^i_{L}
	\end{equation}
	
	\item \emph{Case 2B: $\overline{\mp}_a$ is a blue path of $\overline{\mathbb{P}}$.~} There is no level-$i$ edge with both endpoints in $\mx$ since any such edge would have length at most $\adm(\mx)\leq 5\zeta L_i  < L_i/2$ while a level-$i$ edge has length at least $L_i/2$. Let $\mbe$ be an edge with exactly one endpoint ni $\mx$. If $\mbe$ is incident to a \emph{red subpath} broken from a long path, then $\mbe$ is already handled in Case 2a. $\mbe$ cannot be incident to another blue subpath in Step 4B by Claim B. Thus, it remains to consider the case where $\mbe$ is to another light supercluster $\my'$; $\my'$ may be grouped to a bigger supercluster in Step 5A. (Such an edge $\mbe$ is highlighted red in Figure~\ref{fig:longpath-opt}.) If $\my'$ is a supercluster in $\mathbb{X}_2\cup \mathbb{X}_3$, then the weight of $\mbe$ is already bounded in \textbf{Case 1 } above. If $\my'$ belongs to a supercluster $\mz$ in $\mathbb{X}_5$, we use the potential reduction of superclusters in $\mathbb{X}_5$ to bound the weight of edges  incident to \emph{all} superclusters considered in this case as follows.
	
	By Lemma~\ref{lm:Step15WeightOracle}, if we evenly distribute the potential reduction of every Step-5A clusters to their nodes, each gets $\Omega(\epsilon L_i)$ unit of potential. Thus, $\my'$ has $\Delta^i_{L}(\my') = \Omega(|\mv(\my')|
	\epsilon L_i)$ unit of potential reduction from $\mz$. By the same argument in \textbf{Case 1}, the weight of level-$i$ edges incident to  $\my'$ taken to $H_i$ is  $O(\frac{L_i}{\epsilon}) = O(|\mv(\my')|L_i)$ as $|\mv(\my')| = \Omega(\frac{1}{\epsilon})$. That is, the total weight of edges between blue paths in Step 4B and superclusters in Step 5A is at most:
	
	\begin{equation}\label{eq:H5B2}
	O(\frac{1}{\epsilon}) \sum_{\mz \in \mathbb{X}_5}\Delta^i_{L}(\mz) = O(\frac{1}{\epsilon})\Delta^i_{L} 	
	\end{equation}
\end{itemize}


	
Finally, the lemma follows directly from Equations~\eqref{eq:H5B1},~\eqref{eq:H5B2}, and~\eqref{eq:H5B3}.  \qed
\end{proof}

We now  deal with the special case where no cluster is formed in Steps 1-3.
\begin{lemma}\label{lm:pay-5B-exception}  If there is not supercluster formed in Steps 1-3, then $w(H_i) = O(L_i)$.
\end{lemma}
\begin{proof} Since no supercluster is formed in Step 1, $\mv(\mathcal{F}_1) = \mv_i$.
	Since no supercluster is formed in Step 2  $\overline{\mathcal{F}}_2$, 
	  is a  single (long) path $\overline{\mp}$, $\mathcal{B}_{far} = \emptyset$, and hence $\overline{\mf_3} = \overline{\mp}$. Step 4A will not happen and in Step 4B, $\overline{\mp}$ will be broken into subpaths of augmented diameter at least $5\zeta L_i$ and at most $12\zeta L_i$. Since $\mathcal{B}_{far} = \emptyset$ and edges in $\mathcal{B}_{close}$ are not added to $H_i$, any edge $e\in H_i$ (added in Step 5B) must be incident to a red node.  
	
	The augmented distance from any red node to at least one endpoint of $\overline{\mp}$ is at most $L_i$ by definition, and hence there are at most $2(\frac{L_i}{5\zeta  L_i}) = O(1)$ superclusters in Step 4B that are incident to level-$i$ edges. By  Corollary~\ref{cor:deg-C-5B}, there are $O(1)$ edges between any two superclusters. Thus, the total  weight of all edges added to $H_i$ is
	\begin{equation*}
	w(H_i) = O(1) L_i = O(L_i),
	\end{equation*}
	as claimed.\qed
\end{proof}

If there is no supercluster formed in Steps 1-3, then by Lemma~\ref{lm:pay-5B-exception}, $w(H) = O(L_i)$; clearly $\Delta^i_{L}\geq 0$. Otherwise, by Lemmas~\ref{lm:H5A},~\ref{lm:H5B} and~\ref{lm:H5C}, $w(H_i) =  (\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon})\Delta^i_{L}$. Thus, in both cases, we conclude that:
\begin{equation*}
w(H_i) = O(\frac{\wsp_{\mathcal{O}_{G,t}}}{\epsilon})\Delta^i_{L} + O(L_i),
\end{equation*}
as claimed in Theorem~\ref{thm:cluster-opt-t2}.

